On Bellman's Optimality Principle for zs-POSGs

Many non-trivial sequential decision-making problems are efficiently solved by relying on Bellman's optimality principle, i.e., exploiting the fact that sub-problems are nested recursively within the original problem. Here we show how it can apply to (infinite horizon) 2-player zero-sum partially observable stochastic games (zs-POSGs) by (i) taking a central planner's viewpoint, which can only reason on a sufficient statistic called occupancy state, and (ii) turning such problems into zero-sum occupancy Markov games (zs-OMGs). Then, exploiting the Lipschitz-continuity of the value function in occupancy space, one can derive a version of the HSVI algorithm (Heuristic Search Value Iteration) that provably finds an $\epsilon$-Nash equilibrium in finite time.

==> Makefile <==
DEPS_DIR = .deps
LATEXMK = latexmk -recorder -use-make -deps \
	-e 'warn qq(In Makefile, turn off custom dependencies);' \
	-e '@cus_dep_list = ();' \
	-e 'show_cus_dep();'

main.pdf : main.tex Makefile
	if [ ! -e $(DEPS_DIR) ]; then mkdir $(DEPS_DIR); fi
	-$(LATEXMK) -pdf -deps-out=$(DEPS_DIR)/$@P $<
	./clean-deps.sh $(DEPS_DIR)/$@P

clean :
	rm -f *~
	latexmk -c

veryclean:
	rm -rf *~ .deps *.bbl figures/*.bak
	latexmk -C

